LS-CS-residual (LS-CS): Compressive Sensing on Least Squares Residual

We consider the problem of recursively and causally reconstructing time sequences of sparse signals (with unknown and time-varying sparsity patterns) from a limited number of noisy linear measurements. The sparsity pattern is assumed to change slowly with time. The idea of our proposed solution, LS-CS-residual (LS-CS), is to replace compressed sensing (CS) on the observation by CS on the least squares (LS) residual computed using the previous estimate of the support. We bound CS-residual error and show that when the number of available measurements is small, the bound is much smaller than that on CS error if the sparsity pattern changes slowly enough. We also obtain conditions for "stability" of LS-CS over time for a signal model that allows support additions and removals, and that allows coefficients to gradually increase (decrease) until they reach a constant value (become zero). By "stability", we mean that the number of misses and extras in the support estimate remain bounded by time-invariant values (in turn implying a time-invariant bound on LS-CS error). The concept is meaningful only if the bounds are small compared to the support size. Numerical experiments backing our claims are shown.

==> bound_error_8.tex <==

\Section{Bounding CS-residual Error}
\label{csresbound}

We first bound the CS-residual reconstruction error and compare it with the bound on CS error. In Sec. \ref{tightbnd}, we give a tighter bound on the CS-residual error, but which holds under stronger assumptions. All bounds depend on $|T|$, $|\Delta|$.%In the last subsection, we bound the LS-CS error in terms of $|\tT|$, $|\tDelta|$.% for situations where $n$ is small so that Theorems 1.1, 1.2 of \cite{dantzig} do not apply

{\em To simplify notation, in this section, we remove the subscript $t$}. Consider reconstructing $x$ with support, $N$, from $y:=Ax + w$. The support can be written as $N = (T \cup \Delta) \setminus \Delta_e$ where $T$ is the ``known" part of the support (equal to support estimate from the previous time), $\Delta_e := T \setminus N$ and $\Delta:= N \setminus T$.%$\Delta_e := T \setminus N$ is the error in $T$ and $\Delta:= N \setminus T$ is the unknown part.%  a sparse vector,


\Subsection{Bounding CS-residual Error}
\label{csresbound1}
If $n$ is large enough so that $|T|+|\Delta|=|N|+|\Delta_e| \le \sinf$, then we can use the bounds given in Theorems 1.1 or 1.2 of \cite{dantzig} to bound the CS-residual error. But recall that CS-residual is primarily designed for situations where $n$ is smaller. It applies CS to the observation residual $\tilde{y} = A \beta + w$ where $\beta := x - \xhat_{\text{init}}$ is a $(|T|+|\Delta|)$-sparse signal, that is compressible (small) along $T$. To bound its error, we first prove Lemma \ref{thm13} which modifies Theorem 1.3 of \cite{dantzig} to apply it to ``sparse-compressible signals", i.e. sparse signals that are partly (or fully) compressible. Next, we bound $\|\beta_T\|$ (the ``compressible" part of $\beta$). Finally we use this lemma along with the bound on $\|\beta_T\|$ to obtain the CS-residual error bound.%, i.e. signals in which some (or all) nonzero coefficients are roughly at the noise level.

\begin{lemma}[CS error bound - sparse-compressible signal]%[modification of Theorem 1.3 of \cite{dantzig}]%Let $w$ is bounded noise with
Assume that $\|w\|_\infty \le \frac{\lambda}{\|A\|_1}$ (bounded noise). Let $\zeta$ is an $S_{nz}$-sparse vector with support $T_{nz}$, and we measure $y:=A\zeta+w$. Its estimate, $\zetahat$, obtained by solving (\ref{simplecs}), obeys the following.
For all sets $\rest \subseteq T_{nz}$ of size $|\rest|= S_{nz}-S$ and for all $1 \le S \le \min(\sinf,S_{nz})$,
\bea
\label{ell1term}
\|\zeta - \zetahat\|^2 \sle C_2(S) S  \lambda^2 + C_3(S) \frac{\| (\zeta)_{{\rest}} \|_1^2}{S} \nn  \\
\label{ell2term}
\sle C_2(S) S  \lambda^2 + C_3(S) \frac{(S_{nz} - S)}{S} \| (\zeta)_{{\rest}} \|^2,   \nn \\
 \text{where~~} C_2(S) \sdefn \frac{48}{(1-\delta_{2S} - \theta_{S,2S})^2},   \nn \\ % S \sigma_{obs}^2
\text{and~~} C_3(S) \sdefn 8 + \frac{24 \theta_{S,2S}^2}{(1-\delta_{2S} - \theta_{S,2S})^2} % \frac{(S_{nz} - S)}{S} \| (\beta)_{\rest} \|^2 \ \
\label{defc2c3}
\eea
\label{thm13}
\end{lemma}
The proof is given in Appendix \ref{thm13_proof}.
Recall that $\sinf$ is defined in Definition \ref{delta_bnd}.

Recall that $\beta = x - \xhat_{\text{init}}$ can be rewritten as
\bea
\beta_T \se   - ({A_T}'A_T)^{-1} {A_T}'(A_\Delta x_\Delta + w)  \nn \\ %x_T - {A_T}^\dag y =
\beta_\Delta \se x_\Delta, \ \ \ (\beta)_{(T \cup \Delta)^c} = 0
\label{defbeta2}
\eea
As long as $\delta_{|T|}< 1$, $\|\beta_T\|^2$ can be bounded as follows.
\bea
\|\beta_T\|^2 \sle  2  [ \|({A_T}'A_T)^{-1} {A_T}'A_\Delta x_\Delta\|^2 + \|({A_T}'A_T)^{-1} {A_T}' w \|^2 ]   \nn \\
\sle  2 \frac{{\theta_{|T|,|\Delta|}}^2}{(1-\delta_{|T|})^2} \|x_\Delta\|^2 + \frac{2}{(1-\delta_{|T|})} \|w\|^2
\label{betabound}
\eea
The above follows by using (a) $\|({A_T}'A_T)^{-1}{A_T}'\|^2 = \|({A_T}'A_T)^{-1}\| \le 1/(1-\delta_{|T|})$ (if $\delta_{|T|}<1$) and (b) $\|{A_T}'A_\Delta\| \le \theta_{|T|,|\Delta|}$. (a) follows because $\|({A_T}'A_T)^{-1}\|$ is the inverse of the minimum eigenvalue of ${A_T}'A_T$. (b) follows from (\ref{def_theta}) by setting $c_1 = {A_{T_1}}'A_{T_2} c_2$, $T_1 =T$, and $T_2=\Delta$.%
%By setting $c_1 = {A_{T_1}}'A_{T_2} c_2$ in (\ref{def_theta}), it is easy to see that  $\|{A_{T_1}}'A_{T_2}\| \le \theta_{S,S'}$.

From (\ref{betabound}), it is clear that if the noise is small and if $|\Delta|$, $|\Delta_e|$ are small enough so that $\theta$ is small, $\|\beta_T\|$ is small. Using (\ref{betabound}) along with Lemma \ref{thm13}, we can prove the following.%_{|T|,|\Delta|}

\begin{theorem}[CS-residual error bound]
Assume that $|T|:=|N|+|\Delta_e|-|\Delta| \le \sone$ and $\|w\|_\infty \le \frac{\lambda}{\|A\|_1}$. Then,
%The CS-residual reconstruction error, $\|x - \xhat_{\CSres}\|^2$ is bounded by
\bea
&& \| x -\xhat_{\CSres} \|^2 \le  \min_{1 \le S \le \min(\sinf,|T|+|\Delta|)} F_{\CSres}(S)    \nn \\
&& F_{\CSres}(S):= [ C_2(S) S \lambda^2 + C_3(S) \frac{|T|+|\Delta|-S}{S} B(S) ], \nn \\%\ \text{where} \nn \\ %
&& B(S)=\left\{ \begin{array}{ll}
8{\theta}^2 \|x_\Delta\|^2 +  4 \|w\|^2  &  \text{if} \ S \ge |\Delta| \nn \\
8{\theta}^2 \|x_\Delta\|^2 +  4 \|w\|^2 + \|x_\Delta(|\Delta|-S)\|^2  &  \text{if} \  S < |\Delta|
\end{array} \right. \nn \\
%&& \sm := 8{\theta_{|N|+|\Delta_e|-|\Delta|,|\Delta|}}^2 \|x_\Delta\|^2 +  4 \|w\|^2 %\|\beta_T\|_1^2 \sle 2|T| [4{\theta_{|T|,|\Delta|}}^2 \|x_\Delta\|^2 + 2 \|w\|^2]
\label{tighterbnd}
\eea
where $\theta := \theta_{|T|,|\Delta|}$ and $C_2(S)$, $C_3(S)$ are defined in (\ref{defc2c3}).
\label{thm1}
\end{theorem}

The proof is given in Appendix \ref{thm13_proof}. {\em Recall: $x_\Delta(K)$ is the vector containing the $K$ smallest magnitude elements of $x_\Delta$.}% of $x_\Delta$.%

A simple corollary of the above result follows by applying it for a particular value of $S$, $S=|\Delta|$ when $|\Delta| > 0$. This will usually result in the smallest bound in situations where $\sinf$ is not much larger than $|\Delta|$. %Since $|\Delta| \ge 1$, we further simplify the bound by using $|T|/|\Delta| \le |T|$.
When $|\Delta|=0$, $\beta_T = {A_T}^\dag w$ which is anyway quite small. It is not immediately clear which value of $S$ is the best. We retain the $\min$ in this case. We also bound $\|w\|$ by its maximum value, $\sqrt{n}\lambda/\|A\|_1$.%$\|w\|_\infty$ by its maximum value. %, although all values will be small
%This is usually the best since $\|\beta_T\|$ is small and since the constants are strongly increasing functions of $S$ particularly when $S$ approaches $\sinf$.
%We use $S=1$ when $|\Delta|=0$ (all additions have been detected). The constants
\begin{corollary}[simpler CS-residual error bound]%=|N|+|\Delta_e|-|\Delta|
Assume that  $\|w\|_\infty \le {\lambda}/{\|A\|_1}$, $|\Delta| \le \sinf$ and $|T| \le \sone$.
\\ \\
1) {If $|\Delta|>0$}, %$\|x - \xhat_{\CSres}\|^2 \le C' + C''{\theta_{|T|,|\Delta|}}^2 \|x_\Delta\|^2$, where%
\bea
&& \|x - \xhat_{\CSres}\|^2 \le C' + C''{\theta_{|T|,|\Delta|}}^2 \|x_\Delta\|^2, \ \ \text{where} \nn \\
%&& \|x - \xhat_{\CSres}\|^2 \le C' + C''{\theta_{|T|,|\Delta|}}^2 \|x_\Delta\|^2, \ \text{where} \nn \\
%\frac{|T|}{|\Delta|}
&& C' \equiv C'(|T|,|\Delta|) := C_2(|\Delta|) |\Delta| \lambda^2 + 4 C_3(|\Delta|) \frac{|T|}{|\Delta|} \frac{n\lambda^2}{\|A\|_1^2} \nn \\
&& C'' \equiv C''(|T|,|\Delta|) := 8 C_3(|\Delta|) |T| %\frac{|T|}{|\Delta|}
\label{defcprime}
\eea
2) {If $|\Delta|=0$}, $\|x - \xhat_{\CSres}\|^2 \le B_0$ where
\bea
B_{0} := \min_{1 \le S \le \sinf} [ C_2(S) S \lambda^2 + C_3(S) \frac{|T|-S}{S} \frac{4n\lambda^2}{\|A\|_1^2} ] \ \ \ \ \
\label{defB0}
\eea
where $C_2(S)$, $C_3(S)$ are defined in (\ref{defc2c3}).
\label{cor1}
\end{corollary}
This corollary is used in the LS-CS stability result.%
%\bea
%&& C(|\Delta|) + C'(|T|,|\Delta|) + C''(|T|,|\Delta|){\theta_{|T|,|\Delta|}}^2 \|x_\Delta\|^2, \ \text{where} \nn \\
%&& C(S_\Delta) := C_2(S_\Delta) S_\Delta \lambda^2 \nn \\
%&& C'(S_T,S_\Delta) := 4 C_3(S_\Delta) \frac{S_T}{S_\Delta} \frac{n\lambda^2}{\|A\|_1^2} \nn \\
%&& C''(S_T,S_\Delta) := 8 C_3(S_\Delta) \frac{S_T}{S_\Delta}
%\eea

%\begin{remark}
%Notice that $C'(|T|,|\Delta|)$ and $C''(|T|,|\Delta|)$ (and the bound itself) are {\em non-decreasing functions of $|T|$, $|\Delta|$}.
%%$C'(|T|,|\Delta|)$, $C''(|T|,|\Delta|)$ are increasing
%We use the above bound to study stability in Sec. \ref{stability}.%
%\end{remark}

\begin{remark}%, $w \sim \n(0,\sigma^2I)$, (instead of assuming bounded noise)
It is easy to modify the above results for {\em Gaussian noise}, $w \sim \n(0,\sigma^2I)$, in a fashion analogous to the results of \cite{dantzig}. Like  \cite{dantzig}, we will also get ``large probability" results. We do not do this here because any large probability result will make the study of stability over time difficult.%If we use $\lambda=\tilde\lambda \sigma$ in (\ref{simplecs}), then we can claim that the bound of Theorem \ref{thm1}, with $\lambda = \tilde\lambda \sigma$, holds with ``large probability" (same probability as that given in \cite{dantzig}). We do not do this because any large probability result will make the study of stability of over time difficult (the intersection of an infinite number of independent ``large probability" events will still have probability zero).%Lemma \ref{thm13} and Currently using $\lambda = \|A\|_1 \|w\|_\infty$
\end{remark}

\begin{remark}
%This remark responds to a comment by an anonymous reviewer.
In the bounds of Theorem \ref{thm1} or Corollary \ref{cor1}, there is a term that is proportional to $(|T|+|\Delta|-S)$ or to $|T|$ respectively. This comes from Lemma \ref{thm13} when we bound the $\ell_1$ norm term, $\| (\zeta)_{{\rest}} \|_1^2$, by $(S_{nz}-S)$ times $\| (\zeta)_{{\rest}} \|^2$. A similar term is also there in the CS bound given below in (\ref{csbnd}). This is the bound for CS error which holds under the same weak assumptions as those used by our result\footnote{A term containing the $\ell_1$ norm of the ``compressible" part appears in all bounds for CS for compressible signals, e.g. \cite[Thm 1.3]{dantzig}, and hence also appears when we try to bound CS error for sparse signals with not-enough measurements.}.%treat a sparse signal as a ``sparse-compressible" signal.%Since our approach treats the signal residual, $\beta := x - \xhat_{t,\text{init}}$, as a sparse signal that is compressible along $T$, we get this term too.%
\end{remark}

\Subsection{Comparing CS-residual and CS error bounds}
\label{comparecs}
%Since $\beta$ is a $|T \cup \Delta|$ sparse vector with elements of $\beta_T$ being compressible (small) compared to elements of $x_T$, and since $|\Delta|$ is much smaller than $|N|$, it is fair to claim that $\beta$ is approximately much more sparse compared to $x$. This is the key reason CS-residual should outperform CS, particularly when $n$ is small.
We now compare the CS-residual bound with that of CS.
\begin{remark}
By showing that the upper bound on CS-residual error is much smaller, we only show that the performance guarantees for CS-residual are better than those for CS. To actually compare their errors, we use simulations.%demonstrate that CS-residual outperforms CS, we use simulations.
\end{remark}
%We use the following notion of compressibility: a $T \cup \Delta$ sparse vector $\beta$ is compressible along $T$ if $\|\beta_T\| < \|\beta_\Delta\|$, i.e. the norm of the compressible part be smaller than the norm of the un-compressible part.
 %be smaller than the magnitude of any nonzero element of $x$ except the newly added ones (which may be small initially), i.e. we require that $\|\beta_T\|^2 < \min_{i \in (N \setminus \Delta)} x_i^2$.


To compare the CS-residual bound with CS, first note that the CS error bounds for sparse signals given in Theorems 1.1 and 1.2 of \cite{dantzig} apply  only when $\delta_{2S} + \theta_{S,2S} < 1$ holds for $S=|N|$, i.e. when $|N| \le \sinf$. When $n$ is small and this does not hold, these results are not applicable. On the other hand, Lemma \ref{thm13} does not assume anything about $\sinf$. %our result only requires $\delta_{2S} + \theta_{S,2S} < 1$ to hold for $S=|\Delta|$, in addition to requiring that $\delta_{|N|+|\Delta_e|} < 1/2$. To bound CS error only under this assumption, we use Lemma \ref{thm13}.  (and consequently Theorem \ref{thm1})
Let $\xhat_{CS}$ denote the simple CS output. Using Lemma \ref{thm13}, it is easy to see that % $\|x - \xhat_{CS}\|^2$ is bounded by
\bea %\| x -\xhat_{\CSres} \|^2 \sle
&& \|x - \xhat_{CS}\|^2 \le \min_{1 \le S \le \min(\sinf,|N|)} F_{CS}(S) \nn \\
&& F_{CS}(S):=[ C_2(S) S \lambda^2 + C_3(S) \frac{|N|-S}{S} B_{CS}(S) ], \nn \\
&& B_{CS}(S) := \|x_N(|N|-S)\|^2
\label{csbnd}
\eea

Compare (\ref{tighterbnd}) with (\ref{csbnd}) under the following assumptions.
\ben
\item  The magnitude of the largest element of $x_\Delta$ is smaller than or equal to that of the smallest element of $x_{N \setminus \Delta}$, i.e. $|(x_\Delta)_{(1)}| \le |(x_{N\setminus \Delta})_{(N\setminus \Delta)}|$.
% i.e. $\|x_\Delta\|_\infty \le |x_{N\setminus \Delta}(1)|$.
 This is reasonable since $\Delta$ contains the recently added elements which will typically be smaller while ${N \setminus \Delta}$ contains the previously added elements which should have a larger value.% But this assumption also allows magnitude equality of all elements of $x_N$, e.g. if all are always $\pm 1$.
%newly added elements at the current time and the undetected ones from the previous time instant, both of
\label{Delsmall}

\item $|\Delta|$, $|\Delta_e|$ are small enough (i.e. $S_a$ is small enough and $T \approx N_{t-1}$) %(support changes slowly enough and the previous support estimate is accurate enough)
and the noise is small enough so that
\ben
\item $|\Delta| \le |N|/10$, and $|\Delta_e| \le  |N|/10$
%\item $\theta_{|T|,|\Delta|}^2 < \frac{\|x_\Delta\|^2 - 4\|w\|^2}{8\|x_\Delta\|^2}$

\item ${\theta_{|T|,|\Delta|}}^2 < 1/8$, and
 $\|w\|^2 \le \frac{\|x_{N\setminus \Delta}(|\Delta|)\|^2(1-8 \theta^2)}{4}$.%, where $\theta:=\theta_{|T|,|\Delta|}$
\label{noisesmall}
\een
\item $n$ is small so that $\sinf =0.2|N|$, but is just large enough so that $\sone \ge 1.1|N|$ (needed to apply Theorem \ref{thm1}).%
\een
Assumptions \ref{Delsmall} and \ref{noisesmall} ensure that $\|\beta_T\|^2 \le 8{\theta}^2 \|x_\Delta\|^2 +  4 \|w\|^2 \le 8{\theta}^2  \|x_{N \setminus \Delta}(|\Delta|)\|^2 +  4 \|w\|^2 \le \|x_{N \setminus \Delta}(|\Delta|)\|^2$, i.e.  $\beta_T$ is ``compressible enough".%\footnote{One way to quantify compressibility of $\beta$ would be to ask for $\|\beta_T\| < \|\beta_\Delta\|=\|x_\Delta\|$. But $\beta_T = A_T^\dag A_\Delta x_\Delta + A_T^\dag w$. When a new addition just occurs, $\|x_\Delta\|$ may not be greater than the noise level $\|w\|$. Because of assumption \ref{Delsmall} above, $\|x_\Delta\| \le  \|x_{N \setminus \Delta}(|\Delta|)\|$. Thus requiring that $\|\beta_T\| < \|x_{N\setminus \Delta}(|\Delta|)\|$ is a weaker requirement (since $x_{N \setminus \Delta}$ contains the previously added values of $x$ which should have reached a stable state that will be significantly above the noise level).}.

Under the above assumptions, we show that $F_{\CSres}(S)$ in (\ref{tighterbnd}) is significantly smaller than $F_{CS}(S)$ in (\ref{csbnd}) for each value of $S$ and hence the same will hold for the upper bounds\footnote{\label{minS}Notice that $\frac{F_{\CSres}(S)}{F_{CS}(S)} \le a$ for all $S$ implies that $\frac{\min_{S} F_{\CSres}(S)}{F_{CS}(S)} \le a$ for all $S$. Since this holds for all $S$, it also holds for the max taken over $S$, i.e. $\frac{\min_{S} F_{\CSres}(S)}{\min_{S}F_{CS}(S)} = \max_{S} \frac{\min_{S} F_{\CSres}(S)}{F_{CS}(S)} \le a$.}.% which take $\min_{S \le \sinf}$

%(which take a $\min$ over all $S$) \footnote{\label{minS}If $\frac{f_1(S)}{f_2(S)} < a$ for all $S$, then  $\frac{\min_S f_1(S)}{f_2(S)} < a$ for all $S$ and thus $ \max_S \frac{\min_S f_1(S)}{f_2(S)} = \frac{\min_S f_1(S)}{\min_S f_2(S)} < a$. }.

The CS-residual error would typically increase with $|\Delta|$ and $|\Delta_e|$. Thus we compare the CS-residual bound for their largest values, $|\Delta|=0.1|N|= |\Delta_e|$, with the CS bound.% {\em worst case}

For any $S$, the first term in $F_{\CSres}(S)$ and $F_{CS}(S)$ is the same. In the second term, the main difference is in $B(S)$ versus $B_{CS}(S)$. The constants are almost the same, their ratio is $\frac{|N|+|\Delta_e|-S}{|N|-S} = 1+ \frac{|\Delta_e|}{|N|-S} \le 9/8$ (follows by setting $S=\sinf=0.2|N|$ and $|\Delta_e|=0.1|N|$). Thus if we can show that $B(S)$ is much smaller than $B_{CS}(S)$, we will be done.%

First consider $S \in [0.1|N|, 0.2|N|]$. In this case,%follow from $\|x(kS)\|^2 \le k\|x(S)\|^2$, $x_N(0.1|N|)=x_\Delta$ and $\|x_\Delta\| \le \|x_{N \setminus \Delta}(0.1|N|)\|$
\bea
B(S) \se 8{\theta}^2 \|x_\Delta\|^2 +  4 \|w\|^2  \le \|x_{N\setminus \Delta}(0.1|N|)\|^2 \nn \\
%
B_{CS}(S) \sge B_{CS}(0.2|N|) \nn \\
\se \|x_N(0.8|N|)\|^2 =  \|x_\Delta\|^2 + \|x_{N \setminus \Delta} (0.7|N|)\|^2 \nn \\
& > & \|x_{N \setminus \Delta} (0.7|N|)\|^2 \nn \\
\sge 7 \|x_{N \setminus \Delta} (0.1|N|)\|^2 \ge  7 B(S)
\eea
Now consider $S \in [1, 0.1|N|)$.
\bea
B(S) \se 8{\theta}^2 \|x_\Delta\|^2 +  4 \|w\|^2  + \|x_\Delta(0.1|N|-S)\|^2    \nn \\
\sle \|x_{N\setminus \Delta}(0.1|N|)\|^2  + \|x_\Delta\|^2  \nn \\
\sle 2\|x_{N\setminus \Delta}(0.1|N|)\|^2   \nn \\
%
B_{CS}(S) & > & B_{CS}(0.1|N|) = \|x_N(0.9|N|)\|^2 \nn \\
& > & \|x_{N \setminus \Delta} (0.8|N|)\|^2  \nn \\
\sge 8 \|x_{N \setminus \Delta} (0.1|N|)\|^2  \ge 4 B(S)
\eea
Thus $\frac{B(S)}{B_{CS}(S)} \le 1/4$. %for all $S \le \sinf$. %Thus the ratio of the second term of $F_{\CSres}(S)$ to that of $F_{CS}(S)$ is The first terms are the same.
 Denote the common first term in $F_\CSres$ and $F_{CS}$  by $\text{T1}$. Denote the second terms by $\text{T2}_\CSres$ and $\text{T2}_{CS}$. %respectively.
Thus, $\frac{\text{T2}_\CSres}{\text{T2}_{CS}} =  \frac{B(S)}{B_{CS}(S)} \frac{|N|+|\Delta_e|-S}{|N|-S}  \le (1/4) (9/8)=9/32$, for all $S \le \sinf$.  Thus, $F_{\CSres}(S) \le F_{CS}(S)$ for all $S \le \sinf$. By footnote \ref{minS} the same holds for the bounds.%the CS-residual bound, $\min_{S \le \sinf} F_{\CSres}(S)$, is also smaller than the CS bound, $\min_{S \le \sinf} F_{CS}(S)$} (see footnote \ref{minS}).

Furthermore, if the noise is small enough, and for $S \le \sinf$, the second term is the dominant term in $F_{CS}(S)$, i.e. $\text{T1} \ll \text{T2}_{CS}$. Then $\frac{F_{\CSres}(S)}{F_{CS}(S)} = \frac{\text{T1}}{\text{T1}+\text{T2}_{CS}} + \frac{\text{T2}_{\CSres}}{\text{T1}+\text{T2}_{CS}} \approx \frac{\text{T2}_\CSres}{\text{T2}_{CS}} \le 9/32$, i.e. $F_{\CSres}(S)/F_{CS}(S)$ is also roughly less than $9/32$ for all $S$.
From footnote \ref{minS}, this means that the {\em CS-residual bound} also satisfies the same thing, and thus {\em it is significantly smaller.}%is also roughly less than $9/32$ of the CS bound (significantly smaller).%, particularly in $F_{CS}(S)$

If $|\Delta|=0$, assumption \ref{noisesmall}) does not hold and so the above comparison does not hold. But clearly, under high enough SNR, $B_0$ in Corollary \ref{cor1} is much smaller than (\ref{csbnd}).%

\subsubsection{Monte Carlo Comparison}
We compared CS-residual error with CS error using simulations for a single time instant problem with $m=200$, $|N|=20$, $|\Delta|=|\Delta_e|=0.1|N|=2$ and for $n=45,59,100$. Nonzero signal values were $\pm 1$ with equal probability. We compare the normalized MSE's in Table \ref{static_table}. The CS-residual error is much smaller than the CS error except when $n=100$ (large). See Sec. \ref{staticsim} for details.
%To compare LS-CS with CS, simulate all nonzero elements to be $\pm 1$. Simulate 2 time instants, at t=1, use n=m/2, at t=2, use n = 2S(2)-1. take m=256,S=8 at t=1, S = 10 at t=2. Thus n(2)=19, n(1)=128. This simulates mostly zero false adds and 2 new adds. Then use n(1)=56 = 7 log2 m. This simulates some false adds also.


\Subsection{Tighter CS-residual Bound under Stronger Assumptions**}% and $A$ is incoherent enough
\label{tightbnd}
%This section is motivated by a very useful comment of an anonymous reviewer.
To address an anonymous reviewer's comment, we give below a tighter error bound for CS-residual (does not contain a term proportional to $|T|$). But this also holds under a stronger assumption. This section can be skipped in a quick reading.

 Using (\ref{defbeta2}), $\| (\beta)_{T} \|_1 \le \|{A_T}^\dag A_\Delta\|_1 \|x_\Delta\|_1 + \|{A_T}^\dag w\|_1$. Notice that if the noise is small and $|\Delta|$ is small, $\| (\beta)_{T} \|_1$ will be small. In particular, if $\| (\beta)_{T} \|_1 \le b \| x_\Delta \|_1$, by applying the first inequality of Lemma \ref{thm13} with $\zeta = \beta$, $S_{nz}=|T|+|\Delta|$, $S = |\Delta|$ and $\rest=T$; using $\| x_\Delta \|_1\le \sqrt{|\Delta|} \| x_\Delta \|$; and combining the resulting bound with that given in Corollary \ref{cor1}, we get the following.%
\begin{corollary}
Assume that
\ben
\item $\|w\|_\infty \le \frac{\lambda}{\|A\|_1}$, $|\Delta| \le \sinf$, $|T| \le \sone$,
\item  $\|{A_T}^\dag A_\Delta\|_1 < c$ and $\|x_\Delta\|_1 > \frac{\|{A_T}^\dag w\|_1}{b-\|{A_T}^\dag A_\Delta\|_1}$ for a $b>c$%
\label{x_delta_large}
\een
then,
\bea
&& \|x - \xhat_{\CSres}\|^2 \ \le  \ C_2(|\Delta|) |\Delta|  \lambda^2 \ + \ C_3(|\Delta|) \times   \nn \\
&& \min(b^2 \|x_\Delta\|^2, \ {8|T|}{\theta}^2 \|x_\Delta\|^2 + {4|T|} \frac{n\lambda^2}{\|A\|_1^2})
%&& \min(b^2 \|x_\Delta\|^2, \ \frac{8|T|}{|\Delta|}{\theta}^2 \|x_\Delta\|^2 + \frac{4|T|}{|\Delta|} \frac{n\lambda^2}{\|A\|_1^2})
\label{cor2bnd}
\eea
If $|\Delta|=0$,  condition \ref{x_delta_large} cannot hold. In this case, $\|x - \xhat_{\CSres}\|^2 \le B_0$ with $B_0$ defined in Corollary \ref{cor1}.
$\blacksquare$%
\label{cor2}
\end{corollary}

%{|\Delta|}
 Notice that {\em the first term in the $\min$ does not contain ${|T|}$.} The above bound is tighter when this first term is smaller, i.e. $b$ is small enough (happens if  $|\Delta|$ small but $\|x_\Delta\|_\infty$ large).%
%$\frac{b^2}{8\theta^2}\frac{|\Delta|}{|T|} < 1$.% , i.e. when $b$ is small enough $|\Delta_e|$,

%
%\Subsection{A CS-residual Bound under a Stronger Assumption**}% and $A$ is incoherent enough
%This subsection is motivated by a very useful comment of an anonymous reviewer.
%Notice that if we apply the first inequality given in Lemma 1 with $\zeta = \beta$, $S_{nz}=|T|+|\Delta|$, $S = |\Delta|$ and $\rest=T$, we get
%\bea
%\|x - \xhat_{\CSres}\|^2 \sle C_2(|\Delta|) |\Delta|  \lambda^2 + C_3(|\Delta|) \frac{\| (\beta)_{T} \|_1^2}{|\Delta|}
%\label{tbnd}
%\eea
%Now, $\| (\beta)_{T} \|_1 \le \|{A_T}^\dag A_\Delta\|_1 \|x_\Delta\|_1 + \|{A_T}^\dag w\|_1$.
%Assume that $|\Delta|$ is small enough and $A$ is incoherent enough so that $\|{A_T}^\dag A_\Delta\|_1 < c < 1$. If, for some $b > c$, $\|x_\Delta\|_1$ is large enough to satisfy $\|x_\Delta\|_1 \ge \frac{\|{A_T}^\dag w\|_1}{b-\|{A_T}^\dag A_\Delta\|_1}$, then $\| (\beta)_{T} \|_1 \le  b \|x_\Delta\|_1$. Using this and $\|x_\Delta\|_1^2 \le |\Delta| \|x_\Delta\|^2$ in (\ref{tbnd}), we get
%\bea
%\|x - \xhat_{\CSres}\|^2 \sle C_2(|\Delta|) |\Delta|  \lambda^2 + C_3(|\Delta|) b^2 \|x_\Delta\|^2 \nn
%\eea
%%Of course when $|\Delta|=0$, $\|x_\Delta\|_1=0$  and hence the above bound cannot be applied.
%
%Thus, under a stronger assumption, we get the following corollary. Notice that the bound does not contain $\frac{|T|}{|\Delta|}$ in the second term, and thus can be significantly tighter than that of Corollary \ref{cor1} in certain situations,  $\frac{b^2}{8\theta^2}\frac{|\Delta|}{|T|} < 1$.% or Theorem \ref{thm1}
%\begin{corollary}
%Assume that
%\ben
%\item $\|w\|_\infty \le \frac{\lambda}{\|A\|_1}$, $|\Delta| \le \sinf$, $|T| \le \sone$, $\|{A_T}^\dag A_\Delta\|_1 < c$,
%\item for some $b > c$, $\|x_\Delta\|_1 > \frac{\|{A_T}^\dag w\|_1}{b-\|{A_T}^\dag A_\Delta\|_1}$
%\label{x_delta_large}
%\een
%then,
%\bea
%\|x - \xhat_{\CSres}\|^2 \sle C_2(|\Delta|) |\Delta|  \lambda^2 + C_3(|\Delta|)b^2 \|x_\Delta\|^2
%\label{cor2bnd}
%\eea
%%where $C_2(S)$, $C_3(S)$ are defined in Lemma \ref{thm13}.
%If $|\Delta|=0$,  condition \ref{x_delta_large} cannot hold. In this case, $\|x - \xhat_{\CSres}\|^2 \le B_0$ with $B_0$ defined in Corollary \ref{cor1}.
%$\blacksquare$%
%\label{cor2}
%\end{corollary}
%
%%For situations where $\|x_\Delta\|_1$ is not large enough, if we replace $x_\Delta$ by $x_{N\setminus \Delta}$ in condition \ref{x_delta_large} and also assume $\|x_\Delta\|_\infty \le |x_{N\setminus \Delta}(1)|$, then (\ref{cor2bnd}) holds with $x_\Delta$ replaced by $x_{N\setminus \Delta}$.%



%\Subsection{Bounding LS-CS Error**}
%Recall that $\tDelta := N_t \setminus \Nhat_t$, $\tDeltae: = \Nhat_t \setminus N_t$, and $\tT:= \Nhat_t$. If $|\tT| \le \sone$, the LS-CS error is bounded as follows:
%\bea
%\|(x - \xhat)_\tDelta\|^2 \se \|(x)_\tDelta\|^2 \le  |\tDelta| \|x_\tDelta\|_\infty^2 \nn \\
%\|(x - \xhat)_\tT\|^2  \sle 8{\theta_{|\tT|,|\tDelta|}}^2 |\tDelta| \|x_\tDelta\|_\infty^2 + 4\frac{n \lambda^2}{\|A\|_1^2}  %\|w\|^2
%%\sle (1+ 8{\theta_{|\tT|,|\tDelta|}}^2) \|x_\tDelta\|^2 + 4\|w\|^2 \nn \\
%%\sle (1+ 8{\theta_{|\tT|,|\tDelta|}}^2) |\tDelta| \|x_\tDelta\|_\infty^2  + 4\|w\|^2
%\label{lscs_error}
%\eea
%This bound is given here primarily for use in the next section.

%\Subsection{A CS-residual Bound under a Stronger Assumption}% and $A$ is incoherent enough
%This subsection is motivated by a very useful comment of an anonymous reviewer.
%Notice that if we apply the first inequality given in Lemma 1 with $\zeta = \beta$, $S_{nz}=|T|+|\Delta|$, $S = |\Delta|$ and $\rest=T$, we get
%\bea
%\|x - \xhat_{\CSres}\|^2 \sle C_2(|\Delta|) |\Delta|  \lambda^2 + C_3(|\Delta|) \frac{\| (\beta)_{T} \|_1^2}{|\Delta|}
%\label{tbnd}
%\eea
%Now, $\| (\beta)_{T} \|_1 \le \|{A_T}^\dag A_\Delta\|_1 \|x_\Delta\|_1 + \|{A_T}^\dag w\|_1$.
%Assume that $|\Delta|$ is small enough so that $\|{A_T}^\dag A_\Delta\|_1 < 1$. If, in addition, $\|x_\Delta\|_1$ is large enough to satisfy $\|x_\Delta\|_1 \ge \frac{\|{A_T}^\dag w\|_1}{1-\|{A_T}^\dag A_\Delta\|_1}$, then $\| (\beta)_{T} \|_1 \le  \|x_\Delta\|_1$. Also, $\|x_\Delta\|_1^2 \le |\Delta| \|x_\Delta\|^2$.
%Using this in (\ref{tbnd}), we get
%\bea
%\|x - \xhat_{\CSres}\|^2 \sle C_2(|\Delta|) |\Delta|  \lambda^2 + C_3(|\Delta|)\|x_\Delta\|^2
%\eea
%%Of course when $|\Delta|=0$, $\|x_\Delta\|_1=0$  and hence the above bound cannot be applied.
%
%Thus, under a stronger assumption, we get the following corollary. Notice that the bound does not contain $\frac{|T|}{|\Delta|}$ in the second term, and thus may be a tighter bound than that of Corollary \ref{cor1} or Theorem \ref{thm1} in certain situations.
%\begin{corollary}
%Assume that
%\ben
%\item $\|w\|_\infty \le \frac{\lambda}{\|A\|_1}$, $|\Delta| \le \sinf$, $|T| \le \sone$, $\|{A_T}^\dag A_\Delta\|_1 < 1$,
%\item and $\|x_\Delta\|_1 > \frac{\|{A_T}^\dag w\|_1}{1-\|{A_T}^\dag A_\Delta\|_1}$
%\label{x_delta_large}
%\een
%then,
%\bea
%\|x - \xhat_{\CSres}\|^2 \sle C_2(|\Delta|) |\Delta|  \lambda^2 + C_3(|\Delta|) \|x_\Delta\|^2 \nn
%\eea
%%where $C_2(S)$, $C_3(S)$ are defined in Lemma \ref{thm13}.
%If $|\Delta|=0$,  condition \ref{x_delta_large} cannot hold. In this case, $\|x - \xhat_{\CSres}\|^2 \le B_0$ with $B_0$ defined in Corollary \ref{cor1}.
%$\blacksquare$%
%\label{cor2}
%\end{corollary}
%
%A further corollary can be obtained which  is useful when $\|x_\Delta\|_1$ is not large enough. If we replace condition \ref{x_delta_large} in the above corollary by (i) $\|x_\Delta\|_\infty \le |x_{N\setminus \Delta}(1)|$ and (ii) $\|x_{N\setminus \Delta}(|\Delta|)\|_1 \ge \frac{\|{A_T}^\dag w\|_1}{ (1-\|{A_T}^\dag A_\Delta\|_1)}$, then
%$$\|x - \xhat_{\CSres}\|^2 \le C_2(|\Delta|) |\Delta|  \lambda^2 + C_3(|\Delta|)\|x_{N\setminus \Delta}(|\Delta|)\|^2$$
%%, but may still give a tighter bound than Corollary \ref{cor1}


%Define an $\ell_1$ version of $\theta$ and $\delta$. Let $\theta_{S,S',1} := \max_{|T|\le S,|\Delta| \le S'} \|{A_T}'A_\Delta\|_1$. Let $\delta_{S,1}:= \|A_T'A_T\|???$






==> stability_9.tex <==
 %for a given support size,  a given maximum number of additions/deletions per unit time, and a given rate of increase of the  magnitudes of the newly added coefficients,  under what conditions on the measurement model (noise power and $\delta_S, \theta_{S,S'}$) and for what delay between addition times,
\Section{LS-CS Stability}% and $|\tT|,|\tDelta|$ respectively
\label{stability}
So far we bounded CS-residual error as a function of $|T|,|\Delta|$. The bound is small as long as $|\Delta_e|$ and $|\Delta|$ are small.
A similar bound on LS-CS error as a function of $|\tT|,|\tDelta|$ is easy to obtain. The next question is: under what conditions on the measurement model and the signal model (rate of increase of new coefficients and delay between addition times), {\em will LS-CS be stable, i.e. the number of  extras, $|\tDelta_e|$, and the number of misses, $|\tDelta|$, (and hence also $|\Delta_e|$, $|\Delta|$) remain bounded by a small value, compared to the signal support size, at all times}? This, in turn, will imply that the LS-CS error remains bounded by a small value (compared to the signal power). A second question, which helps answer the first, is: when can we claim that  $|\tDelta_e|$, $|\tDelta|$ become zero within a finite delay of a new addition time? %{\em the LS-CS estimate becomes equal to the genie-aided LS estimate within a finite delay after a new addition/removal.} /removal
When $|\tDelta|=0=|\tDelta_e|$, $\Nhat_t = N_t$, and so the LS-CS estimate is equal to the {\em genie-aided LS} estimate (LS estimate computed using the true support, $N_t$).% The genie-LS is the BLUE estimator.%  the true support estimate Assuming finite maximum signal power

\Subsection{Signal Model}
\label{signalmodel}

For studying stability, we need to assume a signal model. We assume the following deterministic model that (a) assumes a nonzero delay between new coefficient addition times, (b) allows a new coefficient magnitude to gradually increase from zero for sometime and finally reach a constant value and (c) allows coefficients to gradually decrease and become zero (get removed from support). At $t=0$, we assume that $x_0$ is $(S_0-S_a)$ sparse with all ``large" coefficients with values $\pm M$.% These have values $\pm M$ with equal

\begin{sigmodel} The model is as follows.
\ben
\item {\em Initialization. } At $t=0$, $x_0$ is $(S_0-S_a)$ sparse. All its nonzero coefficients have values $\pm M$.% We assume that all elements of its support get correctly estimated and there are no false detections, i.e. at $t=1$, $T= \Nhat_0 = N_0$. with equal probability

\item {\em Addition. } At $t=t_j =1+(j-1)d$, for all $j \ge 1$, $S_a$ new coefficients get added. Denote the set of indices of coefficients added at $t=t_j$ by $\add = \add(j)$. A new coefficient, $i \in \add$, gets added at an initial magnitude $a_i$ (its sign can be $\pm1$) and then its magnitude increases at a rate $a_i$ until it either reaches $M$ or for $d$ time units. Thus, the maximum magnitude of the $i^{th}$ coefficient, for $i \notin N_0$, is $\min(M,da_i)$ while that for $i \in N_0$ is $M$.%The sign does not change.  with equal probability
% These coefficients are ``increasing" until $t_{j+1}-1$. %(which are still in the ``increasing phase") by $\add = \add(j)$.

\item {\em Removal. } $S_a$ coefficients get removed at $t=t_{j+1}-1 = jd$ for all $j \ge1$. Denote the set of indices of coefficients which get removed at $t_{j+1}-1$ by $\rem = \rem(j)$. During  $[t_{j+1}-r, t_{j+1}-1]$, the elements of  $\rem$ start to decrease and become zero at $t=t_{j+1}-1$.  For coefficient, $i$, the rate of decrease is $\min(M,da_i)/r$ per unit time.% (the $j=0$ case is included in the initialization)

\item The sets $\add(j)$ and $\rem(j)$ are disjoint, i.e. the coefficients that just got added do not get removed.
\een
Thus at any $t \in [t_j, t_{j+1}-r-1]$, the support can be split as $\add$ {\em (increasing coefficients)} and $N \setminus \add$ {\em (constant coefficients)}, where $N = N_t = N_{t_j}$. At any $t \in [t_{j+1}-r, t_{j+1}-2]$, it can be split as $\add$ (increasing), $\rem$ {\em (decreasing)}, $N \setminus (\add \cup \rem)$ (constant). At $t=t_{j+1}-1$, $N=N_t = N_{t_j} \setminus \rem$ (all constant).%
\label{sigmod1}
\end{sigmodel}

Notice that in the above model the signal support size remains roughly constant. It is $S_0$ or $(S_0-S_a)$ at all times. Also, the maximum signal power is bounded by $S_0M^2$. The minimum signal power is $\sum_{i=0}^{S_0-S_a-1}a_{(m-i)}$. Recall that $a_{(k)}$ denotes the $k^{th}$ largest element of $a$.


\Subsection{Three Key Lemmas}
\label{keylemmas} %, i.e. showing that the number of misses and extras remain bounded by a small enough value compared to signal support size,
Proving stability, i.e. showing that the number of misses, $|\tDelta|$, and extras, $|\tDelta_e|$, remain bounded, requires finding sufficient conditions for the following three things to hold at the current time: (a) one, or a certain number of, large undetected coefficients definitely get detected; (b) large enough detected coefficients definitely do not get falsely deleted, and (c) every-so-often the extras (false detects or true removals) definitely do get deleted. (a) and (b) are used to ensure that $|\tDelta|$ remains bounded while (c) is  used to ensure that $|\tDelta_e|$, and hence $|\tT| \le |N|+|\tDelta_e|$, remains bounded. These three things are done in the following three lemmas.

\begin{lemma}[Detection condition]
Assume that  $|T| \le S_T \le \sone$, $|\Delta| \le S_\Delta \le \sinf$, and  $\|w\|_\infty \le \lambda/\|A\|_1$. %If both inequalities of (\ref{largestdet}) hold, then
The current largest magnitude undetected element, $(x_\Delta)_{(1)}$, will definitely get detected at the current time, if
\bea
&& \max_{|T| \le S_T, |\Delta| \le S_\Delta}  2{\theta_{|T|,|\Delta|}}^2 {|\Delta| C''(|T|,|\Delta|)} < 1, \ \text{and}        \nn \\
&& \max_{|T| \le S_T, |\Delta| \le S_\Delta} \frac{2\alpha^2 + 2C'(|T|,|\Delta|)}{1- 2 \theta_{|T|,|\Delta|}^2 |\Delta| C''(|T|,|\Delta|)}  < (x_\Delta)_{(1)}^2 \ \ \ \ \
\label{largestdet}
\eea
\label{largest}
\end{lemma}


\begin{lemma}[No false deletion condition] % All $i \in \tT_\dett$ with $x_i^2 \ge b_1$
Assume that $\|w\|_\infty \le \lambda/\|A\|_1$, $|\tT_\dett| \le S_T \le \sone$ and $|\tDelta_\dett| \le S_\Delta$. For a given $b_1$, let $T_l:=\{i \in \tT_\dett:x_i^2 \ge b_1\}$. All $i \in T_l$ will not get (falsely) deleted at the current time if
\bea
b_1^2 >2 \alpha_{del}^2 + \frac{8n\lambda^2}{\|A\|_1^2} + 16 {\theta_{S_T,S_\Delta}}^2 |\tDelta_\dett| \|x_{\tDelta_\dett}\|_\infty^2 %\|x_{\tDelta_\dett}\|^2.
\eea
\label{nofalsedelscond}
\end{lemma}

\begin{lemma}[Deletion condition]
Assume that $\|w\|_\infty \le \lambda/\|A\|_1$, $|\tT_\dett| \le S_T \le \sone$ and $|\tDelta_\dett| \le S_\Delta$. All elements of $\tDelta_{e,\dett}$ will get deleted if
\label{truedelscond}
$
\alpha_{del}^2 \ge \frac{4n\lambda^2}{\|A\|_1^2} + 8 {\theta_{S_T,S_\Delta}}^2 |\tDelta_\dett| \|x_{\tDelta_\dett}\|_\infty^2 % \|x_{\tDelta_\dett}\|^2.
$.
\end{lemma}

These lemmas are proved in Appendix \ref{append_lscs_stab_1}. Lemma \ref{largest} follows from Corollary \ref{cor1} and a few simple facts.  Lemmas \ref{nofalsedelscond} and \ref{truedelscond} follow from a simple bound on the error after the detection and LS step.



\Subsection{The Main Result}


\begin{figure}[t!]
\centerline{
%\epsfig{file = stabfig_cor4.eps, width=8cm}
\epsfig{file = stabfig_final_2.eps, width=8cm}
}
%\vspace{-0.1in}
\caption{\small{Our approach to show stability (prove Theorem \ref{stabres}). We split $[t_j,t_{j+1}-1]$ into the four sub-intervals shown above and ensure no false deletion (No-FD) / detection (DET)  / deletion (DEL) of the coefficients listed in each.
%DET: Detect, DEL: Delete, No-FD: No False Deletion.
The notation $\add_{(i)}$ refers to the $i^{th}$ largest increasing coefficient. Recall: in $[t_j,t_{j+1}-r-1]$, $\add$ is the increasing coefficients' set and $N \setminus \add$ is the constant coefficients' set.%
}}
\vspace{-0.2in}
\label{stabfig}
\end{figure}


The LS-CS algorithm is given in Sec. \ref{lscsalgo}. By running simple CS at $t=0$ with an appropriate number of measurements, $n_0 > n$ (usually much larger), we assume that we detect all nonzero coefficients and there are no false detects, i.e. $\Nhat_0 = N_0$. This assumption is made for simplicity, and as we explain later in Remark \ref{initremark}, it is not restrictive.
%so that we can focus on the time sequence. e $S_0-S_a$  (just below the theorem)

For stability, we need to ensure that within a finite delay of a new addition time, all new additions definitely get detected (call this delay the ``detection delay"). This needs to be done while ensuring that there are no false deletions of either the constant or the definitely detected increasing coefficients. Further, by assuming that the delay between two addition times is larger than the ``detection delay" plus the coefficient decrease time, $r$, and by setting the deletion threshold high enough to definitely delete false detects / true removals in the duration after the ``detection delay", we can show stability.% (so that $|\tT|$ remains bounded)

To obtain our result, the above is done by splitting $[t_j, t_{j+1}-1]$ into the four subintervals shown in Fig. \ref{stabfig} and using the lemmas from the previous subsection to find sufficient conditions so that the following hold for some $d_0 < d$:
%and bounding  $|\tDelta|$ and $|\tDelta_e|$ (and hence $|\tT|$) for each. As summarized in Fig. \ref{stabfig}, assume that there exists a $d_0 \le d$ such that
\ben
\item At all $t \in [t_j, t_j+d_0-1]$, there is no false deletion of the constant coefficients (during this time the increasing coefficients may be too small and we do not care if they get detected or not). This ensures that the number of misses do not increase beyond $S_a$.
 %or whether get detected and falsely deleted).%may not get detected or may get detected, but falsely deleted).

\item At $t=t_j+d_0+i-1$, for $i=1,\dots S_a$,  (a) the $i^{th}$ largest increasing coefficient definitely gets detected, and (b)  all constant coefficients and the first $i$ largest increasing coefficients do not get falsely deleted. This ensures that by $t=t_j+d_0+S_a-1$, the number of misses becomes zero, i.e. the ``detection delay" is $d_0+S_a-1$.%

\item  At $t=t_j+d_0+S_a-1$,  all false detects get deleted. This is needed to keep $|T|$ bounded.%Before this, the number of false detects, and thus $|T|$, may keep increasing and this claim bounds that.

\item At all $t \in [t_j+d_0+S_a,t_{j+1}-r-1]$,  (a) the current falsely detected set is immediately deleted and (b) none of the constant or increasing coefficients get falsely deleted.

\item At all $t \in [t_{j+1}-r, t_{j+1}-2]$, (a) the current falsely detected set is deleted and (b) none of the decreasing, constant or increasing coefficients are falsely deleted.
\item At $t_{j+1}-1$, all falsely detected and removed coefficients are deleted and there is no false deletion.
\een

Doing the above leads to the following result.

%We do the above as follows. Also see Fig. \ref{stabfig}. By using the CS-residual bound of Corollary \ref{cor1} and assuming that $\theta^2 < 1/2|\Delta|C''$, we can obtain a sufficient condition under which the current maximum magnitude coefficient, $(x_\Delta)_{(1)}$, will definitely get detected. Assume that the newly added coefficients increase fast enough (their $a_i$'s are large enough) so that (a) within $d_0 < d$ time units, at least the largest of them becomes large enough to definitely get detected; and (b) subsequently at each $t \in [t_j+d_0+1,t_j+d_0+S_a-1]$, the current largest element is large enough to definitely get detected. Further, assume that the delay between addition times, $d \ge d_0+S_a+r$. If, at all $t$, we can prevent the false deletion of all constant coefficients and of all increasing coefficients belonging to the current definitely detected set (this set is empty before $t_j+d_0$), we will ensure that by $t=t_j+d_0+S_a-1$, all true additions are detected and there are no false deletions, i.e. $|\tDelta|=0$. To prevent false deletions, we use the fact that a coefficient will definitely not be falsely deleted if its magnitude is larger than $\alpha_{del}$ plus $||(x_t - \xhat_{t,\dett})_{\tT_\dett}||$. $\xhat_{t,\dett}$ is defined in (\ref{secls}).
%
%A second key point is that true removals or false detects are deleted most easily (with smallest deletion threshold) if this is done when $|\tDelta_{\dett}|=0$ (recall that $\tDelta_\dett$ is the unknown support after the detection step). Lastly, for $t \in [t_{j+1}-r, t_{j+1}-2]$  we need to also prevent false deletions of the decreasing coefficients and ensure their deletion at $t_{j+1}-1$.
%
%Based on the above intuition we get the following result.% Its setting is shown in Fig. \ref{stabfig}.  and Fig. \ref{stabfig}


%the second LS step error (step \ref{addls} of Sec. \ref{lscsalgo}). It can be shown that a
% (largest $i$ elements of $\add(j)$ at $t_j+d_0+i-1$) and of all constant coefficients
%Recall that $\tDelta_\dett$ is the unknown support after the coefficient detection step.
% (defined in Sec. \ref{lscs})
% (recall that $\tDelta_\dett$ is the unknown support after the coefficient detection step)

% all true additions have been detected, i.e. when  (so that the error in second LS step is smallest)

\begin{theorem}[LS-CS Stability]
Under Signal Model \ref{sigmod1}, if there exists a $d_0 < d$, so that the following conditions hold:
\ben
\item {\em (initialization)}  all elements of $x_0$ get correctly detected and there are no false additions, i.e. $\Nhat_0 = N_0$,% at $t=1$, at $t=0$,

\item {\em (algorithm - thresholds)} we set $\alpha_{del} = 2 \sqrt{n} \lambda/\|A\|_1$ and we set $\alpha$ large enough so that there are at most $f$ false detections per unit time,
\label{algo_thresh}

\item {\em (measurement model)}
\label{measmodass}
\ben
\item $\|w\|_\infty \le \lambda/\|A\|_1$, $S_a \le \sinf$, $S_0+f(d_0+S_a) \le \sone$, and
\label{sone_sinf_bnd}
\item $\max_{|T| \le S_T, |\Delta| \le S_\Delta}  {2 |\Delta| C''(|T|,|\Delta|) \theta_{|T|,|\Delta|}}^2 < 1$ with $S_T=S_0+f(d_0+S_a)$, $S_\Delta=S_a$
%(here $\theta$, $C''$ are computed at $|T|,|\Delta|$)
\label{thetabnd}
\een

\item {\em (signal model - ensure additions \& no false deletions of increasing coefficients)}  the following hold for all $i=1, \dots S_a$ and for all $\add = \add(j)$ for all $j$:
\label{additioncond}
\ben
\item $\min(M, (d_0+i) (a_\add)_{(i)} )^2 > \\  \max_{|T| \le S_T, |\Delta| \le S_\Delta} \frac{2\alpha^2 + 2C'(|T|,|\Delta|)}{1- 2(\theta_{|T|,|\Delta|})^2 |\Delta| C''(|T|,|\Delta|)}$,
where \\
$S_T=S_0+f(d_0+i-1)$, $S_\Delta=S_a-i+1$, \\ and
\label{add_incr}

\item $\min(M, (d_0+i) (a_\add)_{(i)} )^2 > 2\alpha_{del}^2  + \\ 16(\theta)^2 (S_a-i) \min(M,(d_0+i) (a_\add)_{(i+1)})^2 + ({8n\lambda^2}/{\|A\|_1^2})$, with $(a_\add)_{(S_a+1)} \equiv 0$ and \\ $\theta$ computed at $S_T=S_0+f(d_0+i)$,  $S_\Delta=S_a-i$
\label{nofd_incr}
\een
%$\theta$, $C'$, $C''$ computed at $|T|,|\Delta|$ %$S_T=S_0+f(d_0+i-1)$, $S_\Delta=S_a-i+1$;
%and

%
%\bea
%\label{add_incr}
%&& \min(M, (d_0+i) (a_\add)_{(i)} )^2 > \frac{2\alpha^2 + 2C'}{1- 2(\theta^a)^2 (S_a-i+1) C''}, \ \text{and} \nn \\
%\label{nofd_incr}
%&& \min(M, (d_0+i) (a_\add)_{(i)} )^2 > 2\alpha_{del}^2  + \nn \\
%&& 16(\theta^d)^2 (S_a-i) \min(M,(d_0+i) (a_\add)_{(i+1)})^2 + \frac{8n\lambda^2}{\|A\|_1^2}
%\eea


\item {\em (signal model - ensure no false deletions of constant coefficients)}
 $\min(M,d \min_i a_i)^2 > 2\alpha_{del}^2  + 16 {\theta}^2 S_a  \min(M,(d_0+S_a) \max_i a_i)^2 + ({8n\lambda^2}/{\|A\|_1^2})$, with $\theta$ computed at $S_T=S_0+f(d_0+S_a)$, $S_\Delta=S_a$
\label{nofd_const}

\item {\em (signal model - ensure no false deletions of decreasing coefficients)}  $\min(M,d \min_i a_i)^2 > r^2
(2\alpha_{del}^2 +  \frac{4n\lambda^2}{\|A\|_1^2})$
%(\alpha_{del} +  \frac{2\sqrt{n}\lambda}{\|A\|_1})^2$
\label{nofd_decr}

\item {\em (signal model - delay between addition times large enough)}  $d \ge d_0 + S_a + r$
\label{dlarge}

%
%\bea
%&& \min(M,d \min_i a_i)^2 > \max(G3, 2\alpha_{del}^2  + 2G4) \nn \\
%&& \text{where~} G3: = r^2 (\alpha_{del} +  \frac{2\sqrt{n}\lambda}{\|A\|_1})^2, \text{~and} \nn \\
%&& G4: = 8 {\theta}^2 S_a  \min(M,(d_0+S_a) \max_i a_i)^2 + \frac{4n\lambda^2}{\|A\|_1^2} \ \ \ \ \
%%
%%\min(M,(d_0+S_a-1)  \min_i a_i) >  \alpha_{del} + 2 \frac{\sqrt{n}\lambda}{\|A\|_1} \ \ \ \ \label{nofalsedel_0}
%\label{stable_req}
%\eea

\een
where $C'$, $C''$ are defined in (\ref{defcprime}), then,
\ben
%\item  For $t \in [t_j, t_{j+1}-2]$, $|N| = S_0$ and for $t = t_{j+1}-1$, $|N|=S_0-S_a$.%

\item At all $t$, $|\tDelta| \le S_a$, $|\tDelta_e| \le f(S_a+d_0)$ and $|\tT| \le S_0+f(S_a+d_0)$. The same bounds also hold for $|\Delta|, |\Delta_e|, |T|$ respectively.
%$|\Delta| \le S_a$, $|\Delta_e| \le f(S_a+d_0)$ and $|T| \le S_0+f(S_a+d_0)$. %

\item For all $t \in [t_j+d_0+S_a-1, t_{j+1}-1]$, $\Nhat_t = N_t$, i.e. $|\tDelta|=0 = |\tDelta_e|$ and $|\tT|=|N_t|$.
\een
\label{stabres}
\end{theorem}

The proof is given in Appendix  \ref{append_lscs_stab_2}. %It follows by proving that if the conditions of the theorem hold, then each of the six claims given earlier holds.
{\em Note that in $\min_i a_i$, the $\min$ is taken over $i \in [1,m]$ and same for $\max_i a_i$.}
%
We now give a simple corollary of Theorem \ref{stabres} (proved in Appendix \ref{corproof}).
\begin{corollary}
If the conditions given in Theorem \ref{stabres} hold,
\ben
\item At all $t$, the LS-CS error satisfies %, $\|x_t - \xhat_{t}\|^2$, is bounded by
\bea
\|(x_t - \xhat_{t})_{\tDelta}\|^2  \sle S_a  \min(M, (d_0+S_a)\max_i a_i)^2 \nn \\
\|(x_t - \xhat_{t})_{\tT}\|^2 \sle   8 {\theta}^2 S_a  \min(M, (d_0+S_a) \max_i a_i)^2  + \nn \\ && 4 \frac{n\lambda^2}{\|A\|_1^2}
\label{lscs_err_max}
\eea
with $\theta$ computed at $S_T=S_0+f(d_0+S_a)$, $S_\Delta=S_a$.

\item At all $t$, the CS-residual error is bounded by %\|x_t - \xhat_{t,\CSres}\|^2 \sle
\bea
\max(B_0,  C' +  {\theta}^2 C'' S_a  \min(M,(d_0+S_a) \max_i a_i)^2  )  \ \ \ \ \
\label{csres_err_max}
\eea
with $\theta, C', C''$ computed at $S_T=S_0+f(d_0+S_a)$, $S_\Delta=S_a$, and $B_0$ is defined in (\ref{defB0}).

%\item For all $t \in [t_j+d_0+S_a-1, t_{j+1}-1]$, the LS-CS estimate is equal the genie-aided LS estimate.% and thus its error is bounded by $4n \lambda^2/\|A\|_1^2$. The CS-residual error is bounded by $B_0$ (defined in Corollary \ref{cor1}).
\een
\label{stabres_cor}
\end{corollary}
%The proof is given in Appendix \ref{corproof}.

\begin{remark}
Note that the initialization assumption is not restrictive. Denote the bound given by Theorem 1.1 of \cite{dantzig} for $S=S_0-S_a$ by $B1$. It is easy to see that this assumption will hold if the addition threshold at $t=0$ is $\alpha_{init}=\sqrt{B1}$ (ensures no false detects) and if $M > \alpha_{init} + \sqrt{B1}=2\sqrt{B1}$ (ensures all true adds detected). If the noise is small enough, by choosing $n_0$ large enough, we can make $B1$ small enough.%
\\
Even if this cannot be done, our result will only change slightly. The misses can be combined with the new additions at $t=1$. Extras will at most increase the bound on $|T|$ by $f$.%%Notice that the initialization assumption is not restrictive. The misses, if any, at $t=0$ can be treated the same way as new additions at $t=1$. Extra additions, if any, at $t=0$ will at most increase the bound on $|T|$ by $f$., if any, at $t=0$
\label{initremark}% at $t=0$ , if any,
\end{remark}

\begin{remark}
By using Corollary \ref{cor2}, instead of Corollary \ref{cor1}, as the starting point for proving the above result, it should be possible to weaken conditions \ref{thetabnd} and \ref{add_incr}. We have not done this here, in order to convey the basic idea in a simpler fashion.% But the discussion will get messier.
\end{remark}%tightening the bound of Corollary \ref{cor1} or by

%Or in other words, for smaller elements,  %Or in other words, when there are fewer unknown coefficients, typically they will get detected at smaller values. %This makes  (\ref{addition_req}) easier to satisfy as more coefficients get detected.%

%strongly increasing functions of $i$, e.g. all terms that depend on  $|\Delta|=S_a-i+1$ will decrease a lot as $|\Delta|$ goes from $S_a$ to $1$. Or in other words, this means that if there are fewer unknown coefficients, typically they will get detected at smaller values. We say ``typically" because there is also a dependence on $|T|$ which, for simplicity, is masked in the upper bounds we take (we have used the largest value reached by $|T|$).


\Subsection{Implications of Theorem \ref{stabres}} %, (\ref{stable_req}) addition and deletion
\label{implications}
Notice that Signal Model \ref{sigmod1} results in {\em bounded SNR and roughly constant signal support size} at all times. Theorem \ref{stabres} and Corollary \ref{stabres_cor} show that, under Signal Model \ref{sigmod1} and under the initialization assumption (made only for simplicity), if
\ben
\item the noise is bounded and $n$ is large enough so that condition \ref{measmodass} holds,
\item the addition/deletion thresholds are appropriately set (condition \ref{algo_thresh}),
\item for a given noise bound and $n$, the smallest rate of coefficient magnitude increase is large enough (condition \ref{additioncond}) and the smallest constant coefficient magnitude is also large enough (conditions \ref{nofd_const}, \ref{nofd_decr}),
\item and the delay between addition times is larger than the ``detection delay" (which in turn depends on the magnitude increase rate), i.e. condition \ref{dlarge} holds,
\een
then,
\ben
\item the number of misses, $|\tDelta| \le S_a$, and the number of extras, $|\tDelta_e| \le f(S_a+d_0)$ and the same bounds hold for $|\Delta|$, $|\Delta_e|$ (where $d_0 \le d$ is the smallest integer for which the conditions of Theorem \ref{stabres} hold);
\item within a finite ``detection delay", $d_0+S_a-1$, all the new additions will definitely get detected and not falsely deleted, and the extras deleted, so that the LS-CS estimate will become equal to the genie-aided LS estimate; and
\item the LS-CS error and the CS-residual step errors are also bounded by time-invariant values.
\een

From  the problem definition section (Assumption \ref{initass}), $S_a  \ll  S_0$. Typically it is easy to choose thresholds such that the average $f$ is small, often even less than 1. Assuming a fast enough signal increase, $d_0$ will also be small.  Thus, with these mild extra assumptions, we can claim that $|\tDelta|$ and $|\tDelta_e|$ will be bounded by a small value compared to the signal support size, i.e. ``stability" is meaningful.

Compare our result to the CS error bound of \cite{dantzig}, which needs $2S_0 \le \sinf$. Typically $\sinf$ is smaller than $\sone$. Compare this to condition \ref{measmodadd}. If the signal increase rate is large enough to ensure that $d_0$ is small enough, this ensures that both conditions\ref{sone_sinf_bnd} and \ref{thetabnd} hold for a much smaller $n$ than what is needed by CS.
% are much weaker than th

Finally notice that we make a slightly restrictive assumption by requiring that the support changes occur every $d$ time instants (although as can be seen from Fig ?, this does hold for the 90\% support change of the cardiac sequence). But we need this assumption in order to answer our second question: when will LS-CS become equal to genie-LS. If we do not care about answering this, we can assume a signal model with $d=1$ and
modify the techniques in this paper to still ensure stability, even though the support estimation errors cannot be shown to become zero. We do this in \cite{icassp10}. 




%. A direct corollary is that the LS-CS error and the CS-residual error are also small.% and also $|\Delta|$ and $|\Delta_e|$,
%Thus $|\tDelta_e|$ is also small compared to $S_0$.

% Thus,  if the thresholds are appropriately set; if the noise is bounded and if there are enough measurements (for a given $S_a$) so that (a) $\sone, \sinf$ satisfy assumption \ref{measmodass} given in Theorem \ref{stabres}, and (b) $\theta^2$, $C',C''$ are small enough, for a given magnitude increase/decrease rate, for (\ref{thetabnd}), (\ref{addition_req}), (\ref{stable_req}) to hold; and if the delay between addition times is large enough for a given magnitude increase/decrease rate, i.e. if $d\ge d_0+S_a+r$, then ``stability" is ensured. By stability, we mean that $|\Delta|$, $|\Delta_e|$ remain bounded by small enough values compared to the signal support size\footnote{Notice that $|\Delta| \le S_a$. From Assumption \ref{initass} of Sec. \ref{probdef}, $S_a  \ll  S_0$. Also $|\Delta_e| \le f(S_a+d_0)$. Typically it is easy to choose thresholds such that the average $f$ is small, often even less than 1. Assuming a fast enough signal increase, $d_0$ is also small. Thus $|\Delta_e|$ is also small compared to $S_0$.}. This, in turn, implies that LS-CS error remains small. Our result also shows that within a finite delay of an addition time, $|\tDelta|$, $|\tDelta_e|$ become zero, i.e. $\Nhat_t = N_t$.  We show an example in Fig. \ref{stability_fig}.%, Sec. \ref{stabsims}.% at all times

%Also, we can compare the worst-case CS-residual bound of (\ref{csres_err_max}) with the worst-case bound for CS.

%One can again compare the CS-residual bound from Corollary \ref{stabres_cor} with that of CS and show that it will be smaller.%

% Let $\sinf=S_a$, $\sone=S_0+f(d_0+S_a)$ and (\ref{thetabnd}) holds. Compare the worst-case CS-residual bound from (\ref{csres_err_max}) with that of CS. In (\ref{csbnd}), $B_{CS}(S_a) \le (S_0-S_a) \min(M,d \max_i a_i)^2$. This is larger than $ S_a  {\theta}^2 \min(M,(d_0+S_a) \max_i a_i)^2$ (we are again comparing upper bounds).% for $S=S_a$.B_{CS}(S) \le

%bounded by a small value.%
%compared to the signal power %\footnote{The sum of the bounds in (\ref{lscs_err_max}) is approximately less than $2S_a M^2$, assuming large enough SNR. Since $S_a  \ll S_0$, this is much smaller than $S_0 M^2$, which is the maximum signal power. The same can be claimed for signal power at a given time, by also bounding LS-CS error at that time.}.
%(if $M$ is approx equal to the average of $da_i$ over all $i$). \|(x_t)_{N_t}\|^2 \le , i.e. $d > d_0 + S_a -1$,
% from our initial assumption , i.e. LS-CS estimate equals genie-LS estimate

\Subsection{Extensions of the Stability Result}
\label{stabres_extensions}

If $r$ is large (slow rate of decrease),  condition \ref{nofd_decr} becomes difficult to satisfy. If we remove this condition, we may not be able to prevent false deletion of the decreasing coefficients when they become too small (go below $\alpha_{del}+\frac{2\sqrt{n}\lambda}{\|A\|_1}$). But since they are small, this will increase  the CS-residual error at the next time instant only slightly. With small changes to our arguments, it should be possible to still prove stability.%the LS-CS error, or

An {\em important modification} of our result studies the case of $d=1$, i.e. when additions/removals occur at every time. In ongoing work \cite{icassp10}, we are able to show stability in this case, although the misses and extras may not become zero. The key idea is to ensure that all coefficients larger than a certain magnitude are always definitely detected and not falsely deleted, and that the false detects/true removals are always immediately deleted.

%A more illustrative and simpler sufficient condition for assumption \ref{additioncond} in Theorem \ref{stabres} follows using $(a_\add)_{(i+1)} \le (a_\add)_{(i)}$.%in (\ref{addition_req}).%
%\begin{corollary}
%Assumption \ref{additioncond} of Theorem \ref{stabres} holds if $\min(M, (d_0+i) (a_\add)_{(i)} )^2 > \max(G1, G5)$ where
%$$G5:= \frac{2\alpha_{del}^2  + {8n\lambda^2}/{\|A\|_1^2}}{1-8(\theta^d)^2 (S_a-i)}$$
%and $G1$ is defined in (\ref{addition_req}).
%This condition, in turn, holds if $\min(M, (d_0+i) a_{(m-S_a+i)}) > \max(G1, G5)$.%
%\end{corollary}
%Notice that $\max(G1, G5)$ is an increasing function of $(S_a-i)$, $|\Delta|$ and  $|T|$. As $i$ increases from 1 to $S_a$, $(S_a-i+1)$ and $|\Delta|$ decrease from $S_a$ to 0 (significant decrease) while the increase in $|T|$ is a small fraction of its initial value. Thus, typically, $\max(G1, G5)$ decreases very fast as $i$ increases. In other words, as the unknown support size, $|\Delta|$, reduces, detection becomes guaranteed at smaller coefficient magnitudes.% typically %from $S_0+fd_0$ to $S_0+f(d_0+S_a-1)$. Notice that a sufficient condition for (\ref{addition_req}) to hold is that $\min(M, (d_0+i) (a_\add)_{(i)} )^2 > \max(G1, G5)$ where $G5:= \frac{2\alpha_{del}^2  + {8n\lambda^2}/{\|A\|_1^2}}{1-8(\theta^d)^2 (S_a-i)}$.



%Various interesting extensions of our result are possible. One is the case when additions occur at every time, i.e. $d=1$. If all new coefficients get added at large enough values, e.g. if $a_i=M$, and if $r=1$, it should be possible to show that all additions will also get detected immediately, thus ensuring stability. We should be able to show stability even if only some get added at large values, while the rest are small (increase slowly). This will require a larger lower bound on $\sinf$.% also


%This is valid only if we get the other bound for deletion step.
%Notice that the RHS of (\ref{addition_req}) is an increasing function of $|T|$, $|\Delta|$. As $i$ increases, $|T|$ increases from $S_0+fd_0$ to $S_0+f(d_0+S_a-1)$ and $|\Delta|$ decreases from $S_a$ to 0. The maximum increase in $|T|$ is $fS_a$ which is a small fraction of  its initial value while the decrease in $|\Delta|$ is much more significant. Thus, typically the right hand side of (\ref{addition_req}) decreases very fast as $i$ increases. In other words, as $|\Delta|$ reduces, typically detection becomes guaranteed at smaller coefficient magnitudes.%, $S_0+fd_0$,


%If we relax the upper bound on $|\Delta|$ to $2S_a$, it should even be possible to handle slow removals (Signal Model \ref{sigmod2}) without requiring either of the above extra assumptions.% (instead of $S_a$) to be at most $2S_a$


% A more interesting case is when only some get added at large values, e.g. if at any given time only a fixed number of the elements of the current $\Delta$ are ``large" while the rest are small (undetectable but also contribute little to the error).
%Another case of interest is when $d=1$ but at any given time only a fixed number of the elements of the current $\Delta$ are ``large" while the rest are small (undetectable but also contribute little to the error).%
%In a simpler case, if all new coefficient magnitudes are equal and large enough to immediately get detected, e.g. if all get added at value $\pm M$, one could still get $d=1$ (additions at every $t$) almost directly from our result (removals will have to be handled differently).
%Removals at every $t$ are even easier to handle. (by slightly modifying the current proof)







